X-Fi: A Modality-Invariant Foundation Model for Multimodal Human Sensing

Human sensing, which employs various sensors and advanced deep learning technologies to accurately capture and interpret human body information, has significantly impacted fields like public security and robotics. However, current human sensing primarily depends on modalities such as cameras and LiDAR, each of which has its own strengths and limitations. Furthermore, existing multi-modal fusion solutions are typically designed for fixed modality combinations, requiring extensive retraining when modalities are added or removed for diverse scenarios. In this paper, we propose a modality-invariant foundation model for all modalities, X-Fi, to address this issue. X-Fi enables the independent or combinatory use of sensor modalities without additional training by utilizing a transformer structure to accommodate variable input sizes and incorporating a novel "X-fusion" mechanism to preserve modality-specific features during multimodal integration. This approach not only enhances adaptability but also facilitates the learning of complementary features across modalities. Extensive experiments conducted on the MM-Fi and XRF55 datasets, employing six distinct modalities, demonstrate that X-Fi achieves state-of-the-art performance in human pose estimation (HPE) and human activity recognition (HAR) tasks. The findings indicate that our proposed model can efficiently support a wide range of human sensing applications, ultimately contributing to the evolution of scalable, multimodal sensing technologies.

==> tables/1.MMFi_result.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[t]
\vspace{-4.3mm}
\centering
\scalebox{0.91}{
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{tabular}{c|ccc|ccc|ccc}
\toprule
\multirow{2}{*}[-2pt]{MM-Fi}            & \multicolumn{3}{|c}{HAR}                            & \multicolumn{6}{|c}{HPE}                                                                             \\ \cmidrule{2-10}
                  & \multicolumn{3}{|c}{Accuracy (\%)}                  & \multicolumn{3}{|c}{MPJPE (mm)}                   & \multicolumn{3}{|c}{PA-MPJPE (mm)}                \\ \midrule
Method          & Baseline & X-Fi   & Imp $\uparrow$                            & Baseline & X-Fi  & Imp $\downarrow$                          & Baseline & X-Fi  & Imp $\downarrow$                          \\ \midrule
I                 & 25.3     & 26.5   & {\color[HTML]{34A853} 1.2\%}   & 141.5    & 93.9  & {\color[HTML]{34A853} 33.6\%} & 66.1     & 60.3  & {\color[HTML]{34A853} 8.9\%}  \\
D                 & 49.9     & 48.1   & {\color[HTML]{FF7F7F} -1.8\%}  & 102.4    & 101.8 & {\color[HTML]{34A853} 0.6\%}  & 52.7     & 48.4  & {\color[HTML]{34A853} 8.2\%}  \\
L                 & 63.9     & 52.7   & {\color[HTML]{FF7F7F} -11.2\%} & 161.3    & 167.1 & {\color[HTML]{FF7F7F} -3.6\%} & 103.5    & 103.2 & {\color[HTML]{34A853} 0.3\%}  \\
R                 & 85.0     & 85.7   & {\color[HTML]{34A853} 0.7\%}   & 141.3    & 127.4 & {\color[HTML]{34A853} 9.8\%}  & 72.4     & 69.8  & {\color[HTML]{34A853} 3.7\%}  \\
W                 & -        & -      & -       & 227.1    & 225.6 & {\color[HTML]{34A853} 0.7\%}  & 107.9    & 105.3 & {\color[HTML]{34A853} 2.5\%}  \\ \midrule
I+D             & 45.2   & 45.3 & {\color[HTML]{34A853} 0.1\%}   & 109.2    & 86.1  & {\color[HTML]{34A853} 21.2\%} & 57.1     & 48.1  & {\color[HTML]{34A853} 15.6\%} \\
I+L             & 23.8   & 35.2 & {\color[HTML]{34A853} 11.4\%}   & 121.2    & 93.0  & {\color[HTML]{34A853} 23.3\%} & 73.0     & 59.7  & {\color[HTML]{34A853} 18.2\%} \\
I+R             & 66.9   & 73.4 & {\color[HTML]{34A853} 6.5\%}   & 140.6    & 88.8  & {\color[HTML]{34A853} 36.8\%} & 68.2     & 57.3  & {\color[HTML]{34A853} 16.0\%} \\
D+L             & 49.7  & 51.6 & {\color[HTML]{34A853} 1.9\%}  & 108.0    & 102.5 & {\color[HTML]{34A853} 5.1\%}  & 55.8     & 48.4  & {\color[HTML]{34A853} 13.3\%} \\
D+R             & 74.1  & 79.8 & {\color[HTML]{34A853} 5.7\%}   & 116.4    & 98.0  & {\color[HTML]{34A853} 15.8\%} & 57.0     & 47.3  & {\color[HTML]{34A853} 17.0\%} \\
L+R             & 85.6   & 88.7 & {\color[HTML]{34A853} 3.1\%}   & 137.0    & 109.8 & {\color[HTML]{34A853} 19.9\%} & 71.9     & 63.4  & {\color[HTML]{34A853} 11.8\%} \\
I+W             & -        & -      & -                              & 156.7    & 93.0  & {\color[HTML]{34A853} 40.7\%} & 86.3     & 59.5  & {\color[HTML]{34A853} 31.1\%} \\
D+W             & -        & -      & -                              & 155.5    & 101.8 & {\color[HTML]{34A853} 34.5\%} & 81.5     & 48.1  & {\color[HTML]{34A853} 41.0\%} \\
L+W             & -        & -      & -                              & 206.2    & 159.5 & {\color[HTML]{34A853} 22.6\%} & 109.3    & 102.7 & {\color[HTML]{34A853} 6.0\%}  \\
R+W             & -        & -      & -                              & 141.3    & 117.2 & {\color[HTML]{34A853} 17.0\%} & 77.6     & 62.7  & {\color[HTML]{34A853} 19.1\%} \\ \midrule
I+D+L         & 43.0   & 48.7 & {\color[HTML]{34A853} 5.7\%}   & 104.5    & 84.8  & {\color[HTML]{34A853} 18.8\%} & 61.2     & 48.2  & {\color[HTML]{34A853} 21.4\%} \\
I+D+R         & 69.1   & 70.7 & {\color[HTML]{34A853} 1.6\%}   & 113.4    & 83.4  & {\color[HTML]{34A853} 26.5\%} & 58.0     & 47.3  & {\color[HTML]{34A853} 18.4\%} \\
I+L+R         & 68.2   & 77.8 & {\color[HTML]{34A853} 9.6\%}   & 135.0    & 88.4  & {\color[HTML]{34A853} 34.5\%} & 67.7     & 57.2  & {\color[HTML]{34A853} 15.6\%} \\
D+L+R         & 72.9   & 80.5 & {\color[HTML]{34A853} 7.6\%}   & 111.3    & 96.0  & {\color[HTML]{34A853} 13.7\%} & 58.4     & 47.3  & {\color[HTML]{34A853} 19.0\%} \\
I+D+W         & -        & -      & -       & 137.8    & 85.3  & {\color[HTML]{34A853} 38.1\%} & 75.3     & 48.1  & {\color[HTML]{34A853} 36.1\%} \\
I+L+W         & -        & -      & -       & 156.2    & 93.0  & {\color[HTML]{34A853} 40.5\%} & 84.8     & 59.7  & {\color[HTML]{34A853} 29.6\%} \\
I+R+W         & -        & -      & -       & 128.9    & 88.5  & {\color[HTML]{34A853} 31.3\%} & 75.0     & 57.1  & {\color[HTML]{34A853} 23.9\%} \\
D+L+W         & -        & -      & -       & 154.6    & 102.0 & {\color[HTML]{34A853} 34.0\%} & 84.1     & 48.1  & {\color[HTML]{34A853} 42.8\%} \\
D+R+W         & -        & -      & -       & 132.0    & 97.0  & {\color[HTML]{34A853} 26.5\%} & 71.8     & 47.1  & {\color[HTML]{34A853} 34.3\%} \\
L+R+W         & -        & -      & -       & 141.6    & 107.4 & {\color[HTML]{34A853} 24.1\%} & 77.0     & 63.1  & {\color[HTML]{34A853} 18.1\%} \\ \midrule
I+D+L+R     & 72.6   & 72.2 & {\color[HTML]{FF7F7F} -0.4\%}  & 109.4    & 83.5  & {\color[HTML]{34A853} 23.6\%} & 61.6     & 47.6  & {\color[HTML]{34A853} 22.8\%} \\
I+D+L+W     & -        & -      & {\color[HTML]{34A853} -}       & 134.6    & 86.0  & {\color[HTML]{34A853} 36.2\%} & 75.4     & 48.2  & {\color[HTML]{34A853} 36.0\%} \\
I+D+R+W     & -        & -      & {\color[HTML]{34A853} -}       & 128.6    & 84.0  & {\color[HTML]{34A853} 34.7\%} & 71.3     & 47.6  & {\color[HTML]{34A853} 33.3\%} \\
I+L+R+W     & -        & -      & {\color[HTML]{34A853} -}       & 174.6    & 88.6  & {\color[HTML]{34A853} 49.2\%} & 78.1     & 57.1  & {\color[HTML]{34A853} 26.8\%} \\
D+L+R+W     & -        & -      & {\color[HTML]{34A853} -}       & 147.6    & 97.6  & {\color[HTML]{34A853} 33.9\%} & 73.1     & 47.4  & {\color[HTML]{34A853} 35.1\%} \\ \midrule
I+D+L+R+W & -        & -      & {\color[HTML]{34A853} -}       & 128.9    & 83.7  & {\color[HTML]{34A853} 35.1\%} & 72.5     & 47.6  & {\color[HTML]{34A853} 34.3\%} \\ \bottomrule
\end{tabular}
}
\vspace{-2mm}
\caption{Performance comparisons of X-Fi with baseline method on MM-Fi dataset. 
% Input modalities are denoted as I (Image), D (Depth), R (mmWave Radar), L (Lidar) and W (WiFi CSI). We assess the performance through MPJPE and PA-MPJPE for HPE task, and accuracy for HAR task. 
Imp denotes the improvement achieved over baseline in percentage level.} \label{tab:mmfi_result_table}
\vspace{-6mm}
\end{table}

==> tables/2.XRF55_result.tex <==
\begin{wraptable}{r}{5.5cm}
\vspace{-4.5mm}
\caption{HAR performance on XRF55.} \label{tab:xrf55_result_table}
\vspace{-3mm}
\scalebox{0.85}{
\begin{tabular}{c|ccc}
\toprule
XRF55    & \multicolumn{3}{c}{Accuracy (\%)} \\ \midrule
Method & Baseline   & X-Fi     & Imp $\uparrow$      \\ \midrule
R        & 82.1\%     & 83.9\%   & {\color[HTML]{34A853} 1.8\%}     \\ 
W        & 77.8\%     & 55.7\%   & {\color[HTML]{FF7F7F} -22.1\%}   \\ 
RF       & 42.2\%     & 42.5\%   & {\color[HTML]{34A853}0.3\%}     \\ \midrule
R+W      & 86.8\%     & 88.2\%   & {\color[HTML]{34A853}1.4\%}     \\ 
R+RF     & 71.4\%     & 86.5\%   & {\color[HTML]{34A853}15.1\%}    \\ 
W+RF     & 55.6\%     & 58.1\%   & {\color[HTML]{34A853}2.5\%}     \\ \midrule
R+W+RF   & 70.6\%     & 89.8\%   & {\color[HTML]{34A853}19.2\%}  \\ \bottomrule
\end{tabular}}
\vspace{-3mm}
\end{wraptable} 

% \begin{minipage}{\textwidth}

% \scalebox{.9}{
% \begin{minipage}[b]{0.445\textwidth}
% % \makeatletter\def\@captype{table}
% \begin{tabular}[h]{c|ccc}
% \toprule
% XRF55    & \multicolumn{3}{c}{Accuracy (\%)} \\ \midrule
% Method & baseline   & X-Fi     & Imp $\uparrow$      \\ \midrule
% R        & 82.1\%     & 83.9\%   & {\color[HTML]{34A853} 1.9\%}     \\ 
% W        & 77.8\%     & 55.7\%   & {\color[HTML]{FF7F7F} -22.1\%}   \\ 
% RF       & 42.2\%     & 42.5\%   & {\color[HTML]{34A853}0.3\%}     \\ \midrule
% R+W      & 86.8\%     & 88.2\%   & {\color[HTML]{34A853}1.4\%}     \\ 
% R+RF     & 71.4\%     & 86.5\%   & {\color[HTML]{34A853}15.1\%}    \\ 
% W+RF     & 55.6\%     & 58.1\%   & {\color[HTML]{34A853}2.6\%}     \\ \midrule
% R+W+RF   & 70.6\%     & 89.8\%   & {\color[HTML]{34A853}19.2\%}  \\ \bottomrule
% \end{tabular}
% % \vspace{5pt}
% \captionof{table}{Performance comparisons of X-Fi with baseline method on XRF55 dataset for HAR task. Input modalities are denoted as R (mmWave Radar), W (WiFi CSI) and RF (RFID).} \label{tab:xrf55_result_table}
% % \vspace{-6mm}
% \end{minipage}
% }
% \scalebox{.9}{
% \begin{minipage}[b]{0.445\textwidth}
% % \makeatletter\def\@captype{table}
% \begin{tabular}[h]{c|ccc}
% \toprule
% XRF55       & \multicolumn{3}{c}{Accuracy (\%)}                      \\ \midrule
% (\(P_{R}\),\(P_{W}\),\(P_{RF}\)) & S1 & S2 & S3 \\ \midrule
% R           & 82.2\%           & 82.4\%           & \textbf{83.9\%}  \\
% W           & 29.1\%           & 37.4\%           & \textbf{55.7\%}  \\
% RF          & 41.6\%           & 41.9\%           & \textbf{42.5\%}  \\ \midrule
% R+W         & 85.1\%           & 86.0\%           & \textbf{88.2\%}  \\
% R+RF        & 84.5\%           & 84.8\%           & \textbf{86.5\%}  \\
% W+RF        & 50.3\%           & 52.7\%           & \textbf{58.1\%}  \\ \midrule
% R+W+RF      & 86.4\%           & 87.3\%           & \textbf{89.8\%} \\ \bottomrule
% \end{tabular}
% % \vspace{5pt}
% \captionof{table}{Performance comparisons of X-Fi trained with varying modality existence lists on the XRF55 dataset for the HAR task.} \label{tab:exist_list_result_table}
% % \vspace{-6mm}
% \end{minipage}
% }
% \scalebox{.5}{
% \begin{minipage}[b]{0.445\textwidth}
% \begin{tabular}{c|cc|cc}
% \toprule
% MM-Fi     & \multicolumn{2}{c|}{MPJPE (mm)} & \multicolumn{2}{c}{PA-MPJPE (mm)} \\ \midrule
% Method    & Transformer  & X-Fusion        & Transformer    & X-Fusion         \\ \midrule
% I         & 99.6         & \textbf{93.9}   & 65.0           & \textbf{60.3}    \\
% L         & 212.2        & \textbf{167.1}  & 109.6          & \textbf{103.2}   \\
% R         & 138.0        & \textbf{127.4}  & 74.6           & \textbf{69.8}    \\
% W         & 243.3        & \textbf{225.6}  & 112.9          & \textbf{105.3}   \\ \midrule
% L + R     & 123.4        & \textbf{109.8}  & 69.9           & \textbf{63.4}    \\
% L + W     & 216.3        & \textbf{159.5}  & 112.7          & \textbf{102.7}   \\ \midrule
% I + L + W & 96.6         & \textbf{93.0}   & 61.5           & \textbf{59.7}   \\ \bottomrule
% \end{tabular}
% % \vspace{5pt}
% \captionof{table}{Comparison between transformer-based fusion and X-Fusion.} \label{tab:transformer_result_table}
% % \vspace{-6mm}
% \end{minipage}
% }
% \vspace{-5mm}
% \end{minipage}

% \begin{table}[b]
% \scalebox{0.78}{
% \begin{tabular}{c|cc|cc}
% \toprule
% MM-Fi     & \multicolumn{2}{c|}{MPJPE (mm)} & \multicolumn{2}{c}{PA-MPJPE (mm)} \\ \midrule
% Method    & Transformer  & X-Fusion        & Transformer    & X-Fusion         \\ \midrule
% I         & 99.6         & \textbf{93.9}   & 65.0           & \textbf{60.3}    \\
% D         & 109.0        & \textbf{101.8}  & 56.1           & \textbf{48.4}    \\
% L         & 212.2        & \textbf{167.1}  & 109.6          & \textbf{103.2}   \\
% R         & 138.0        & \textbf{127.4}  & 74.6           & \textbf{69.8}    \\
% W         & 243.3        & \textbf{225.6}  & 112.9          & \textbf{105.3}   \\ \midrule
% L + R     & 123.4        & \textbf{109.8}  & 69.9           & \textbf{63.4}    \\
% L + W     & 216.3        & \textbf{159.5}  & 112.7          & \textbf{102.7}   \\ \midrule
% I + L + W & 96.6         & \textbf{93.0}   & 61.5           & \textbf{59.7}   \\ \bottomrule
% \end{tabular} }
% \caption{Comparison between transformer-based fusion and X-Fusion.} \label{tab:transformer_result_table}
% \end{table}

% \begin{table}[]
% \scalebox{.87}{\parbox{.43\linewidth}{
% \centering
% \begin{tabular}[]{c|ccc}
% \toprule
% XRF55    & \multicolumn{3}{c}{Accuracy (\%)} \\ \midrule
% modality & baseline   & X-Fi     & Imp $\uparrow$      \\ \midrule
% R        & 82.1\%     & 83.9\%   & {\color[HTML]{34A853} 1.9\%}     \\ 
% W        & 77.8\%     & 55.7\%   & {\color[HTML]{FF7F7F} -22.1\%}   \\ 
% RF       & 42.2\%     & 42.5\%   & {\color[HTML]{34A853}0.3\%}     \\ \midrule
% R+W      & 86.8\%     & 88.2\%   & {\color[HTML]{34A853}1.4\%}     \\ 
% R+RF     & 71.4\%     & 86.5\%   & {\color[HTML]{34A853}15.1\%}    \\ 
% W+RF     & 55.6\%     & 58.1\%   & {\color[HTML]{34A853}2.6\%}     \\ \midrule
% R+W+RF   & 70.6\%     & 89.8\%   & {\color[HTML]{34A853}19.2\%}  \\ \bottomrule
% \end{tabular}
% \vspace{5pt}
% \caption{Performance comparisons of X-Fi with baseline method on XRF dataset for HAR task. Input modalities are denoted as R (mmWave Radar), W (WiFi CSI) and RF (RFID).} \label{tab:xrf55_result_table}
% \vspace{-6mm}
% }}
% \hfill
% \scalebox{.87}{\parbox{.68\linewidth}{
% \centering
% \begin{tabular}[]{c|ccc}
% \toprule
% XRF55       & \multicolumn{3}{c}{Accuracy (\%)}                      \\ \midrule
% (\(P_{R}\),\(P_{W}\),\(P_{RF}\)) & (0.5, 0.5, 0.8) & (0.5, 0.7, 0.7) & (0.5, 0.9, 0.6) \\ \midrule
% R           & 82.2\%           & 82.4\%           & \textbf{83.9\%}  \\
% W           & 29.1\%           & 37.4\%           & \textbf{55.7\%}  \\
% RF          & 41.6\%           & 41.9\%           & \textbf{42.5\%}  \\ \midrule
% R+W         & 85.1\%           & 86.0\%           & \textbf{88.2\%}  \\
% R+RF        & 84.5\%           & 84.8\%           & \textbf{86.5\%}  \\
% W+RF        & 50.3\%           & 52.7\%           & \textbf{58.1\%}  \\ \midrule
% R+W+RF      & 86.4\%           & 87.3\%           & \textbf{89.8\%} \\ \bottomrule
% \end{tabular}
% \vspace{5pt}
% \caption{Performance comparisons of X-Fi training with different modality existence list on XRF dataset for HAR task.} \label{tab:exist_list_result_table}
% \vspace{-6mm}
% }}
% \end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%   Single modality existence list table   %%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{table}[]
% \begin{tabular}{c|ccc}
% \toprule
% XRF55       & \multicolumn{3}{c}{Accuracy (\%)}                      \\ \midrule
% (\(P_{R}\),\(P_{W}\),\(P_{RF}\)) & (0.5, 0.5, 0.8) & (0.5, 0.7, 0.7) & (0.5, 0.9, 0.6) \\ \midrule
% R           & 82.2\%           & 82.4\%           & \textbf{83.9\%}  \\
% W           & 29.1\%           & 37.4\%           & \textbf{55.7\%}  \\
% RF          & 41.6\%           & 41.9\%           & \textbf{42.5\%}  \\ \midrule
% R+W         & 85.1\%           & 86.0\%           & \textbf{88.2\%}  \\
% R+RF        & 84.5\%           & 84.8\%           & \textbf{86.5\%}  \\
% W+RF        & 50.3\%           & 52.7\%           & \textbf{58.1\%}  \\ \midrule
% R+W+RF      & 86.4\%           & 87.3\%           & \textbf{89.8\%} \\ \bottomrule
% \end{tabular}
% \vspace{5pt}
% \caption{Performance comparisons of X-Fi training with different modality existence list on XRF dataset for HAR task.} \label{tab:exist_list_result_table}
% \vspace{-6mm}
% \end{table}

==> tables/3.modality_existence_list_result.tex <==
\begin{wraptable}{r}{5.5cm}
\vspace{-4.3mm}
\caption{Comparisons of X-Fi trained with different modality existence lists.}
\label{tab:exist_list_result_table}
\vspace{-3mm}
\scalebox{0.80}{
\begin{tabular}{c|ccc}
\toprule
XRF55       & \multicolumn{3}{c}{Accuracy (\%)}                      \\ \midrule
(\(P_{R}\),\(P_{W}\),\(P_{RF}\)) & S1 & S2 & S3 \\ \midrule
R           & 82.2\%           & 82.4\%           & \textbf{83.9\%}  \\
W           & 29.1\%           & 37.4\%           & \textbf{55.7\%}  \\
RF          & 41.6\%           & 41.9\%           & \textbf{42.5\%}  \\ \midrule
R+W         & 85.1\%           & 86.0\%           & \textbf{88.2\%}  \\
R+RF        & 84.5\%           & 84.8\%           & \textbf{86.5\%}  \\
W+RF        & 50.3\%           & 52.7\%           & \textbf{58.1\%}  \\ \midrule
R+W+RF      & 86.4\%           & 87.3\%           & \textbf{89.8\%} \\ \bottomrule
\end{tabular}}
\vspace{-4mm}
\end{wraptable} 

==> tables/4.Transformer_result.tex <==
% \begin{wraptable}{r}{5.5cm}
% \caption{A wrapped table going nicely inside the text.}\label{wrap-tab:1}
% \begin{tabular}{ccc}\\\toprule  
% Header-1 & Header-1 & Header-1 \\\midrule
% 2 &3 & 5\\  \midrule
% 2 &3 & 5\\  \midrule
% 2 &3 & 5\\  \bottomrule
% \end{tabular}
% \end{wraptable} 


\begin{wraptable}{r}{6.5cm}
\vspace{-4.3mm}
\caption{Comparison between transformer-based fusion and X-Fusion.} \label{tab:transformer_result_table}
\vspace{-3mm}
\scalebox{0.66}{
\begin{tabular}{c|cc|cc}
\toprule
MM-Fi     & \multicolumn{2}{c|}{MPJPE (mm)} & \multicolumn{2}{c}{PA-MPJPE (mm)} \\ \midrule
Method    & Transformer  & X-Fusion        & Transformer    & X-Fusion         \\ \midrule
I         & 99.6         & \textbf{93.9}   & 65.0           & \textbf{60.3}    \\
D         & 109.0        & \textbf{101.8}  & 56.1           & \textbf{48.4}    \\
L         & 212.2        & \textbf{167.1}  & 109.6          & \textbf{103.2}   \\
R         & 138.0        & \textbf{127.4}  & 74.6           & \textbf{69.8}    \\
W         & 243.3        & \textbf{225.6}  & 112.9          & \textbf{105.3}   \\ \midrule
L + R     & 123.4        & \textbf{109.8}  & 69.9           & \textbf{63.4}    \\
L + W     & 216.3        & \textbf{159.5}  & 112.7          & \textbf{102.7}   \\ \midrule
I + L + W & 96.6         & \textbf{93.0}   & 61.5           & \textbf{59.7}   \\ \bottomrule
\end{tabular} }
\vspace{-4mm}
\end{wraptable} 


% \begin{table}[b]
% \scalebox{0.78}{
% \begin{tabular}{c|cc|cc}
% \toprule
% MM-Fi     & \multicolumn{2}{c|}{MPJPE (mm)} & \multicolumn{2}{c}{PA-MPJPE (mm)} \\ \midrule
% Method    & Transformer  & X-Fusion        & Transformer    & X-Fusion         \\ \midrule
% I         & 99.6         & \textbf{93.9}   & 65.0           & \textbf{60.3}    \\
% D         & 109.0        & \textbf{101.8}  & 56.1           & \textbf{48.4}    \\
% L         & 212.2        & \textbf{167.1}  & 109.6          & \textbf{103.2}   \\
% R         & 138.0        & \textbf{127.4}  & 74.6           & \textbf{69.8}    \\
% W         & 243.3        & \textbf{225.6}  & 112.9          & \textbf{105.3}   \\ \midrule
% L + R     & 123.4        & \textbf{109.8}  & 69.9           & \textbf{63.4}    \\
% L + W     & 216.3        & \textbf{159.5}  & 112.7          & \textbf{102.7}   \\ \midrule
% I + L + W & 96.6         & \textbf{93.0}   & 61.5           & \textbf{59.7}   \\ \bottomrule
% % MM-Fi             & \multicolumn{3}{c|}{MPJPE (mm)}                        & \multicolumn{3}{c}{PA-MPJPE (mm)}                     \\ \midrule
% % Method          & Transformer & \begin{tabular}[c]{@{}c@{}}X-Fusion\\ (iterative)\end{tabular} & \begin{tabular}[c]{@{}c@{}}X-Fusion\\ (stacked)\end{tabular} & Transformer & \begin{tabular}[c]{@{}c@{}}X-Fusion\\ (iterative)\end{tabular} & \begin{tabular}[c]{@{}c@{}}X-Fusion\\ (stacked)\end{tabular} \\ \midrule
% % I                 & 99.6        & \textbf{93.9}       & 100.6             & 65.0        & \textbf{60.3}       & 62.2              \\
% % D                 & 109.0       & 101.8               & \textbf{94.8}     & 56.1        & \textbf{48.4}       & 50.8              \\
% % L                 & 212.2       & \textbf{167.1}      & 184.9             & 109.6       & \textbf{103.2}      & 104.7             \\
% % R                 & 138.0       & 127.4               & \textbf{121.2}    & 74.6        & 69.8                & \textbf{65.4}     \\
% % W                 & 243.3       & \textbf{225.6}      & 229.7             & 112.9       & \textbf{105.3}      & 105.4             \\ \midrule
% % I + D             & 89.7        & 86.1                & \textbf{81.1}     & 52.9        & 48.1                & \textbf{50.0}     \\
% % L + R             & 123.4       & \textbf{109.8}      & 115.5             & 69.9        & \textbf{63.4}       & 64.1              \\
% % L + W             & 216.3       & \textbf{159.5}      & 181.7             & 112.7       & \textbf{102.7}      & 103.9             \\ \midrule
% % I + D + L         & 86.8        & 84.8                & \textbf{78.6}     & 52.2        & \textbf{48.2}       & 49.3              \\
% % I + D + R         & 85.2        & 83.4                & \textbf{78.2}     & 50.9        & \textbf{47.3}       & 48.7              \\
% % I + D + W         & 85.6        & 85.3                & \textbf{79.6}     & 51.5        & \textbf{48.1}       & 49.3              \\ \midrule
% % I + L + R + W     & 93.9        & \textbf{88.6}       & 92.7              & 59.1        & 57.1                & \textbf{56.8}     \\ \midrule
% % I + D + L + R + W & 82.9        & 83.7                & \textbf{76.6}     & 51.3        & \textbf{47.6}       & 47.9              \\ \bottomrule
% \end{tabular} }
% % \vspace{5pt}
% \caption{Comparison between transformer-based fusion and X-Fusion.} \label{tab:transformer_result_table}
% % \caption{Comparison between transformer-based fusion, iterative X-fusion, and stacked X-fusion.} \label{tab:variants_result_table}
% \end{table}

% \begin{table}[b]
% \scalebox{0.78}{
% \begin{tabular}{c|cc|cc}
% \toprule
% MM-Fi     & \multicolumn{2}{c|}{MPJPE (mm)} & \multicolumn{2}{c}{PA-MPJPE (mm)} \\ \midrule
% Method    & Transformer  & X-Fusion        & Transformer    & X-Fusion         \\ \midrule
% I         & 99.6         & \textbf{93.9}   & 65.0           & \textbf{60.3}    \\
% D         & 109.0        & \textbf{101.8}  & 56.1           & \textbf{48.4}    \\
% L         & 212.2        & \textbf{167.1}  & 109.6          & \textbf{103.2}   \\
% R         & 138.0        & \textbf{127.4}  & 74.6           & \textbf{69.8}    \\
% W         & 243.3        & \textbf{225.6}  & 112.9          & \textbf{105.3}   \\ \midrule
% L + R     & 123.4        & \textbf{109.8}  & 69.9           & \textbf{63.4}    \\
% L + W     & 216.3        & \textbf{159.5}  & 112.7          & \textbf{102.7}   \\ \midrule
% I + L + W & 96.6         & \textbf{93.0}   & 61.5           & \textbf{59.7}   \\ \bottomrule
% \end{tabular} }
% % \vspace{5pt}
% \caption{Comparison between transformer-based fusion and X-Fusion.} \label{tab:transformer_result_table}
% \end{table}

